Ultra-High Dimensional Sparse Representations with Binarization for Efficient Text Retrieval

The semantic matching capabilities of neural information retrieval can ameliorate synonymy and polysemy problems of symbolic approaches. However, neural models' dense representations are more suitable for re-ranking, due to their inefficiency. Sparse representations, either in symbolic or latent form, are more efficient with an inverted index. Taking the merits of the sparse and dense representations, we propose an ultra-high dimensional (UHD) representation scheme equipped with directly controllable sparsity. UHD's large capacity and minimal noise and interference among the dimensions allow for binarized representations, which are highly efficient for storage and search. Also proposed is a bucketing method, where the embeddings from multiple layers of BERT are selected/merged to represent diverse linguistic aspects. We test our models with MS MARCO and TREC CAR, showing that our models outperforms other sparse models

==> old_latency.tex <==
\subsection{Analysis on Efficiency (WIP)}
\label{sec::4.6_analysis on efficiency}

\begin{table}
\begin{center}
\begin{tabular}{cccccc}
\toprule
\textbf{n} & \textbf{$\times$0.5} & \textbf{$\times$1} & \textbf{$\times$2} & \textbf{$\times$5} & \textbf{$\times$10} \\ \midrule
\textbf{k=8} & 293.6 &  178.5 & 88.6 & 46.9 & 22.8 \\ 
\textbf{k=16} & & 607.5 & 299.3 & 120.2 & 66.0\\ 
\textbf{k=32} &  &  & & &  \\ 
\bottomrule
\end{tabular}
\end{center}
\caption{Latency (ms) according to the total dimensionality (n$\times$1=81,920) and non-zero dimension size (k) on the MSMARCO Passage Retrieval dev set.}
\label{table:efficiency}
\end{table}

Due to its sparse nature, the proposed UHD-BERT can utilize an in-memory inverted index, which allows efficient and relatively GPU-free retrieval. The efficiency of retrieval using inverted index depends on two factors, $n$ (total dimensionality) and $k$ (number of non-zero dimensions). For each non-zero dimension of queries (equivalent for query term in traditional IR), we have to access documents which have the corresponding dimension activated and their scores. Therefore, the efficiency of the model can be expressed as follows.

\[O(q_k * avg_{dim}) = O(q_k * d_k / n)\]

where $q_k$ is $k$ for queries, $d_k$ is $k$ for documents, and $avg_{dim}$ is number of active documents per dimension. Since we set $q_k$ as a constant (Section \ref{sec::4.3_Symbolic}), the above equation can be expressed more simply.

\begin{equation}
    O(q_k * d_k / n) = O(k / n)
    \label{eq:efficiency}
\end{equation}

According to Eq.\ref{eq:efficiency}, $n$ increases the efficiency while $k$ decreases it. Since increasing $n$ and $k$ helps improve effectiveness (Section \ref{sec::4.4_dimensionality}), improving $n$ and $k$ together would be the best way, but there are different restrictions on the size of the two factors. $k$ determines the amount of information in the in-memory inverted-index, which affects memory usage. $n$ determines the size of the Winner-Take-All module, which affects the GPU usage during training. Due to this restrictions and our limited computing resources, we had to set maximum $n$=81,920 and $k$=16 for the in-memory inverted index. However, to analyze the effects of n and k more extensively, we estimate the latency at larger n and k by either artificially moving (increase $n$) or duplicating (increase $k$) the active dimension to a new dimension. 

Table \ref{table:efficiency} shows latency using the in-memory inverted index for each query according to various $n$ and $k$, where $n$ greater than 81,920 and k greater than 16 are estimations. Latency includes query preprocessing, query encoding, document scoring, and document sorting. Document preprocessing, encoding and inverted index construction can be done offline in advance, so they are not included. The results clearly support the effects of $n$ and $k$ on the efficiency as in Eq.\ref{eq:efficiency}. WAITING FOR RESULTS

Although it was impossible to increase $n$ further (>81,920) with our computing resources, model training with greater $n$ will be possible at the industrial level. The rapid development of GPU devices will further increase the usability of our proposed UHD-BERT model, as increasing $n$ enhance both efficiency and effectiveness. Increasing k also helps improve effectiveness, however, this should take into account the trade-off between effectiveness and efficiency. 
